Zero-sum Stochastic Games with Asymmetric Information

A general model for zero-sum stochastic games with asymmetric information is considered. In this model, each player's information at each time can be divided into a common information part and a private information part. Under certain conditions on the evolution of the common and private information, a dynamic programming characterization of the value of the game (if it exists) is presented. If the value of the zero-sum game does not exist, then the dynamic program provides bounds on the upper and lower values of the game. This dynamic program is then used for a class of zero-sum stochastic games with complete information on one side and partial information on the other, that is, games where one player has complete information about state, actions and observation history while the other player may only have partial information about the state and action history. For such games, it is shown that the value exists and can be characterized using the dynamic program. It is further shown that for this class of games, the dynamic program can be used to compute an equilibrium strategy for the more informed player in which the player selects its action using its private information and the common information belief.

==> appJ_v1.tex <==
%%%%%%%%OLD Version of App J%%%%%%%%%%%%%%%%%%%%%5
\section{Proof of Lemma \ref{structlemma}}\label{structlemmaproof}


%Suppose $h^1$ is any equilibrium strategy for player 1 (we know one exists due to Proposition \ref{kuhnremark}). Since we are dealing with a zero-sum game, we know that (a)  $h^1$ achieves the infimum in $\inf_{g^1 \in \mathcal{G}^1}\sup_{g^2 \in \mathcal{G}^2}J(g^1,g^2)$, (b) any strategy achieving the infimum in the above inf-sup problem will be an equilibrium strategy for player 1 \cite{osborne1994course}. 




Consider any arbitrary strategy $g^1$ for player 1. We will first show that there exists a strategy $\bar{g}^1$ for player 1 such that Let $\iota_t^2 = \{u_{1:t-1}^2,y_{1:t}^2\}$ be a realization of player 2's information $I_t^2$. Define the distribution $\Psi_t(\iota_t^2)$ over the space $\prod_{\tau = 1}^t(\X_{\tau} \times \U_{\tau}^1)$ as follows:
\begin{align*}
\Psi_t(\iota_t^2; x_{1:t},u_{1:t}^1) := \Py^{g^1,h^2}[X_{1:t},U^1_{1:t} = (x_{1:t},u_{1:t}^1) \mid I_t^2 = \iota_t^2],
\end{align*}
%\begin{align*}
%&\Psi_t(\iota_t^2; x_{1:t},u_{1:t}^1) := \notag \\
%~~&\Py^{(g^1,openloop)}[X_{1:t},U^1_{1:t} = (x_{1:t},u_{1:t}^1) \mid I_t^2 = \iota_t^2],
%\end{align*}
if $\iota_t^2$ is \emph{feasible}, that is $\Py^{g^1,h^2}[I_t^2 = \iota_t^2] > 0$, under the \emph{open-loop} strategy $h^2 = (u^2_{1:t-1})$ for player 2. Otherwise, define $\Psi_t(\iota_t^2; x_{1:t},u_{1:t}^1)$ to be the uniform
%\begin{align}
%&\Psi_t(\iota_t^2; x_{1:t},u_{1:t}^1) \\
%&= \begin{cases}
%\Py^{g^1,h^2}[X_{1:t},U_{1:t} = x_{1:t},u_{1:t}^1 \mid I_t^2 = \iota_t^2] & \text{if $\iota_t^2$ is feasible under}\\
%&\text{some open-loop $h^2$}\\
%\mathscr{U}(\cdot) & \text{otherwise},
%\end{cases}
%\end{align}
 distribution over the space $\prod_{\tau = 1}^t(\X_{\tau} \times \U_{\tau}^1)$.

\begin{claim}\label{claimJ1}
Let $g^1$ be player 1's strategy and let $g^2$ be an arbitrary strategy for player 2. Then for any realization $x_{1:t},u_{1:t}^1$ of the variables $X_{1:t},U^1_{1:t}$, we have
\begin{align*}
\Py^{g^1,g^2}[X_{1:t},U^1_{1:t} = (x_{1:t},u_{1:t}^1) \mid I_t^2] = \Psi_t(I_t^2; x_{1:t},u_{1:t}^1),
\end{align*}
almost surely.
\end{claim}
\begin{IEEEproof}
\blue{From player 2's perspective, the system evolution can be seen in the following manner. The system state at time $t$ is $S_t = (X_{1:t},U_{1:t}^1,I^2_t)$. Player 2 obtains a partial observation $Y_{t}^2$ of the state at time $t$. Using information $\{Y_{1:t}^2,U_{1:t-1}^2\}$, player 2 then selects an action $U_t^2$. The state then evolves in a controlled Markovian manner (with dynamics that depend on $g^1$). Thus, from player 2's perspective,  this system is a partially observable Markov decision process (POMDP). The claim then follows from the standard result in POMDPs that the belief on the state given the player's information does not depend on the player's strategy \cite{kumar}.}
%From player 2's perspective, the system evolution can be seen in the following manner. The system state at time $t$ is $S_t = (X_{1:t},U_{1:t}^1,I^2_t)$. Player 2 obtains a partial observation $Y_{t}^2$ at time $t$, which is a function of the system $S_t$, player 2's previous action $U_{t-1}^2$ and an independent noise $W_t^2$ (see equation (\ref{obseq})). Using information $I_t^2 = \{Y_{1:t}^2,U_{1:t-1}^2\}$, player 2 then selects an action $U_t^2$. Because of the dynamics in (\ref{statevol}), this system is a partially observable Markov decision process (POMDP). The claim then follows from the standard result that the belief on the state given the player's information does not depend on the player's strategy in POMDPs \cite{kumar}.
\end{IEEEproof}
%Let the set of \emph{irrelevant variables} be defined as $$\bar{P}_t^1 := \rv{I}_t^1 \setminus (\{X_t\} \cup \rv{I}_t^2) = \{X_{1:t-1},U^1_{1:t-1}\}.$$ 
%Let $x_t$ and $\iota_t^2$ be instances of state $X_t$ and player 2's information $I_t^2$, respectively.

For any instance $\iota_t^2$ of player 2's information $I_t^2$, define the distribution $\Phi_t(\iota_t^2)$ over the space $\X_t \times \U_t^1$ as follows
\begin{align}
\Phi_t(\iota_t^2; x_t, u_t^1) = {\sum_{x_{1:t-1},u_{1:t-1}^1}\Psi_t(\iota_t^2;x_{1:t},u_{1:t}^1)}.
\end{align}
Define strategy $\bar{g}^1$ for player 1 such that for any realization $x_t, \iota_t^2$ of state $X_t$ and player 2's information $I_t^2$ at time $t$, the probability of selecting an action $u_t^1$ at time $t$ is
%\begin{align}
%\bar{h}_t^1(x_t,\iota_{t}^2;u_t^1) &= \sum_{\bar{p}_t^1}\Py^{h^1}[\bar{p}_t^1 \mid x_t,\iota_t^2]h^1_t(\iota_t^1; u_t^1)\\
%&=\sum_{\bar{p}_t^1}\Py^{h^1}[\bar{p}_t^1 \mid x_t,\iota_t^2]\Py^{h^1}[u_t^1 \mid \iota_t^1],
%\end{align}
\begin{align}
&\bar{g}_t^1(x_t,\iota_{t}^2;u_t^1) \\
&= 
\begin{cases}
\frac{\Phi_t(\iota_t^2; x_t,u_t^1)}{\sum_{u_t^{1'}}\Phi_t(\iota_t^2; x_t,u_t^{1'})} & \text{if } \sum_{u_t^{1'}}\Phi_t(\iota_t^2; x_t,u_t^{1'}) > 0\\
\mathscr{U}(\cdot) & \text{otherwise},
\end{cases}
\end{align}
where $\mathscr{U}(\cdot)$ denotes the uniform distribution over the action space $\U_t^1$.

\begin{claim}
For any strategy $g^2$ for player 2, we have
\begin{align*}
\Py^{(g^1,g^2)}[U_t^1 = u_t^1 \mid X_t, I_t^2] = \bar{g}_t^1(X_t,I_{t}^2;u_t^1)
\end{align*}
with probability 1, for every $u_t^1 \in \U_t^1$.
\end{claim}
\begin{IEEEproof}
Let $x_t, \iota_t^2$ be an instance that has a non-zero probability of occurrence under the strategy profile $(g^1,g^2)$. Then using Claim \ref{claimJ1}, we have
\begin{align*}
\Py^{(g^1,g^2)}[X_{1:t},U^1_{1:t} = (x_{1:t},u_{1:t}^1) \mid \iota_t^2] = \Psi_t(\iota_t^2; x_{1:t},u_{1:t}^1),
\end{align*}
for every realization $x_{1:t-1}$ of states $X_{1:t-1}$ and $u_{1:t}^1$ of actions $U_{1:t}^1$. Thus, we have
\begin{align}
\sum_{u_t^{1'}}\Phi_t(\iota_t^2; x_t,u_t^{1'}) = \Py^{(g^1,g^2)}[X_t = x_t \mid I_t^2 = \iota_t^2] > 0.
\end{align}
Therefore, we can say that
\begin{align}
\nonumber\Py^{g^1,g^2}[U_t^1 = u_t^1 \mid X_t = x_t, I_t^2 = \iota_t^2]
&= \frac{\Phi_t(\iota_t^2; x_t,u_t^1)}{\sum_{u_t^{1'}}\Phi_t(\iota_t^2; x_t,u_t^{1'})}\\
&= \bar{g}_t^1(x_t,\iota_{t}^2;u_t^1) .
\end{align}
This concludes the proof of the claim.
\end{IEEEproof}

%\begin{claim}
%The construction of $\bar{g}^1$ does not depend on the strategy $g^2$ of player 2.
%\end{claim}
%\begin{IEEEproof}
%We will first prove by induction that  the conditional distribution $\Py^{g^1,g^2}[I_t^1 \mid I_t^2] = \Py$ does not depend on strategy $g^2$. For induction, assume that this is indeed true upto some time $t$. For an instance $\iota_t^1$ of $I_t^1$, we have
%\begin{align}
%&\nonumber\Py[\iota_{t+1}^1 \mid \iota_{t+1}^2] = \Py[x_{t+1},u_t^1,u_t^2,y_{t+1}^2,I_t^1 \mid \iota_t^2,u_t^2,y_{t+1}^2]\\
%&= \label{g2canc}\frac{\Py[x_{t+1},u_t^1,u_t^2,y_{t+1}^2,\iota_t^1 \mid \iota_t^2]}{\sum_{\bar{x}_{t+1},\bar{u}_t^1,\bar{\iota}_t^1}\Py[\bar{x}_{t+1},\bar{u}_t^1,u_t^2,y_{t+1}^2,\bar{\iota}_t^1 \mid \iota_t^2]}.
%\end{align}
%We have
%\begin{align*}
%&\Py[x_{t+1},u_t^1,u_t^2,y_{t+1}^2,\iota_t^1 \mid \iota_t^2] =  \Py[\iota_t^1 \mid \iota_t^2]g_t^1(\iota_t^1;u_t^1)\\
%&\times g_t^2(\iota_t^2;u_t^2)\Py[x_{t+1} \mid x_t,u_t^1,u_t^2]\Py[y_{t+1}^2\mid x_{t+1},u_t^1,u_t^2].
%\end{align*}
%The only term in this expression that involves the strategy $g_t^2$ is $g_t^2(\iota_t^2;u_t^2)$. In equation (\ref{g2canc}), this term is present in both the numerator and the denominator and thus, it cancels out. Therefore, $\Py^{g^1}[I_{t+1}^1 \mid \iota_{t+1}^2]$ does not depend on the strategy $g^2$ and by induction, this holds for all $t$.
%
%Since $X_t \in I_t^1$, we have that $\Py^{g^1}[I_t^1 \mid x_t,\iota_t^2]$ does not depend on the strategy $g^2$. Lastly, using the fact that the behavioral action $\delta U_t^1 = g_t^1(I_t^1)$, we can conclude that $\Py^{g^1}[U_t^1 = u_t^1 \mid x_t,\iota_t^2]$ does not depend on $g^2$.
%\end{IEEEproof}
\begin{claim}
For any strategy $g^2 \in \mathcal{G}^2$, we have
\[
J(\bar{g}^1,g^2) = J(g^1, g^2).
\]
\end{claim}
\begin{IEEEproof}
To prove this claim, it is sufficient to show that for each time $t$, the triplet $(X_t,U_t^1,U_t^2)$ has the same distribution under strategy profiles $(g^1,g^2)$ and $(\bar{g}^1,g^2)$. This is due to the structure of the cost function $J(\cdot)$ in (\ref{eq:totalcost}). 

For any strategy $g^2 \in \mathcal{G}^2$, we will now prove by induction that at each time $t$, and for any realization of state, actions and player 2's information $x_t,u_t^1,u_t^2, \iota_t^2$, we have
\begin{align}
\label{jointeq}\Py^{g^1,g^2}[x_t,u_t^1,u_t^2,\iota_t^2] = \Py^{\bar{g}^1,g^2}[x_t,u_t^1,u_t^2,\iota_t^2].
\end{align}
For induction, let us assume that this is true at some time $t$. Consider the following
\begin{align}
\label{constarg}&\Py^{g^1,g^2}[x_{t+1},u_{t+1}^1,u_{t+1}^2,\iota_{t+1}^2] \\
&= \nonumber\Py^{g^1,g^2}[x_{t+1},\iota_{t+1}^2]g_t^2(\iota_{t+1}^2;u_{t+1}^2)\Py^{g^1}[u_{t+1}^1\mid x_{t+1},\iota_{t+1}^2]\\
&= \nonumber\Py^{g^1,g^2}[x_{t+1},\iota_{t+1}^2]g_t^2(\iota_{t+1}^2;u_{t+1}^2)\bar{g}_t^1(x_t,\iota_{t}^2;u_t^1)\\
&= \nonumber\Py^{g^1,g^2}[x_{t+1},\iota_{t+1}^2]g_t^2(\iota_{t+1}^2;u_{t+1}^2)\Py^{\bar{g}^1}[u_{t+1}^1\mid x_{t+1},\iota_{t+1}^2].
\end{align}
The last inequality follows from the construction of strategy $\bar{g}^1$. Consider the following
\begin{align}
&\nonumber\Py^{g^1,g^2}[x_{t+1},\iota_{t+1}^2]\\
&= \nonumber\sum_{\bar{x}_t,\bar{u}_t^1}\Py[x_{t+1},\iota_{t+1}^2 \mid \bar{x}_t,\bar{u}_t^1,u_t^2,\iota_t^2]\Py^{g^1,g^2}[\bar{x}_t,\bar{u}_t^1,u_t^1,\iota_t^2]\\
&= \label{indhyp}\sum_{\bar{x}_t,\bar{u}_t^1}\Py[x_{t+1},\iota_{t+1}^2 \mid \bar{x}_t,\bar{u}_t^1,u_t^2,\iota_t^2]\Py^{\bar{g}^1,g^2}[\bar{x}_t,\bar{u}_t^1,u_t^1,\iota_t^2]\\
&=\Py^{\bar{g}^1,g^2}[x_{t+1},\iota_{t+1}^2].
\end{align}
The equality in (\ref{indhyp}) is due to the induction hypothesis. Note that the conditional distribution $\Py[x_{t+1},\iota_{t+1}^2 \mid {x}_t,{u}_t^1,u_t^2,\iota_t^2]$ does not depend on players' strategies (see equations (\ref{statevol}) and (\ref{obseq})). Combining equations (\ref{constarg}) and (\ref{indhyp}), we have
\begin{align*}
\Py^{g^1,g^2}[x_{t+1},u_{t+1}^1,u_{t+1}^2,\iota_{t+1}^2] = \Py^{\bar{g}^1,g^2}[x_{t+1},u_{t+1}^1,u_{t+1}^2,\iota_{t+1}^2].
\end{align*}
Therefore, by induction, this is true for all $t$. This proves our claim.
\end{IEEEproof}
%For any strategy $g^2 \in \mathcal{G}^2$, we will first prove by induction that at each time $t$, and for any realization of state and actions $x_t,u_t^1,u_t^2$, we have
%\begin{align}
%\label{jointeq}\Py^{h^1,g^2}[x_t,u_t^1,u_t^2] = \Py^{\bar{h}^1,g^2}[x_t,u_t^1,u_t^2].
%\end{align}
%Let us make the following induction hypothesis
%\begin{align}
%\Py^{g^1,g^2}[x_t,\iota_t^2] = \Py^{\bar{g}^1,g^2}[x_t,\iota_t^2].
%\end{align}
%This hypothesis is clearly true at $t=1$ because $\bar{P}_1^1 = \varnothing$ and thus, control laws $h_1$ and $\bar{h}^1_1$ are identical. Under the induction hypothesis, we have
%\begin{align}
%&\Py^{g^1,g^2}[x_t,\iota_t^2,u_t^1,u_t^2]\\
%&=\Py^{g^1,g^2}[x_t,\iota_t^2]\Py^{g^2}[u_t^2\mid \iota_t^2]\sum_{\bar{p}_t^1}\Py^{g^1}[\bar{p}_t^1 \mid x_t,\iota_t^2]\\
%&\qquad \qquad \times \Py^{g^1}[u_t^1 \mid \bar{p}_t^1, x_t,\iota_t^2]\\
%& \Py^{g^1,g^2}[x_t,\iota_t^2]\Py^{g^2}[u_t^2\mid \iota_t^2]\Py^{\bar{g}^1}[u_t^1 \mid x_t,\iota_t^2]\\
%&= \Py^{\bar{g}^1,g^2}[x_t,\iota_t^2,u_t^1,u_t^2].
%\end{align}
%We can marginalize $\iota_t^2$ to obtain equality (\ref{jointeq}). We will now prove the induction hypothesis. We have
%\begin{align}
%&\Py^{g^1,g^2}[x_{t+1},\iota_{t+1}^2]\\
%&= \sum_{u_t^1}\Py^{g^1,g^2}[x_{t},\iota_{t}^2,u_t^1,u_t^2]\Py[y_{t+1}^2 \mid x_t,u_t^1,u_t^2,\iota_t^2]\\
%&= \sum_{u_t^1}\Py^{\bar{g}^1,g^2}[x_{t},\iota_{t}^2,u_t^1,u_t^2]\Py[y_{t+1}^2 \mid x_t,u_t^1,u_t^2,\iota_t^2]\\
%&= \Py^{\bar{g}^1,g^2}[x_{t+1},\iota_{t+1}^2].
%\end{align}
%
%\begin{align}
%J(\vct{g}^1,\vct{g}^2)&=\E^{(\vct{h}^1,\vct{g}^2)}\left[\sum_{t=1}^T c_t(\rv{X}_t,\rv{U}_t^{1},\rv{U}_t^2)\right]\\
%&=\sum_{t=1}^T\left[ \E^{(\vct{h}^1,\vct{g}^2)}c_t(\rv{X}_t,\rv{U}_t^{1},\rv{U}_t^2)\right].
%\end{align}



Suppose $h^1$ is any equilibrium strategy for player 1 (we know one exists due to Proposition \ref{kuhnremark}). Since we are dealing with a zero-sum game, we know that (a)  $h^1$ achieves the infimum in $\inf_{g^1 \in \mathcal{G}^1}\sup_{g^2 \in \mathcal{G}^2}J(g^1,g^2)$, (b) any strategy achieving the infimum in the above inf-sup problem will be an equilibrium strategy for player 1 \cite{osborne1994course}. 

Using the equilibrium strategy $h^1$, we can construct a strategy $\bar{h}^1$ as described above such that at each $t$, $\bar{h}_t^1$  uses only the state $\rv{X}_t$ and second player's information $\rv{I}_t^2$ to select its behavioral action \emph{and}
\begin{align*}
\sup_{g^2 \in \mathcal{G}^2}J(\bar{h}^1,g^2) = \sup_{g^2 \in \mathcal{G}^2}J(h^1,g^2) = \inf_{g^1 \in \mathcal{G}^1}\sup_{g^2 \in \mathcal{G}^2}J(g^1,g^2).
\end{align*} 
Thus, $\bar{h}^1$ is an equilibrium strategy for player 1 that uses only the current state and player 2's information.

%%%%%%%%OLD Version of App J%%%%%%%%%%%%%%%%%%%%%5

==> discussion.tex <==
hi

==> gameofteams.tex <==
In this Section, we will formulate a zero-sum game with two \emph{teams} of players and obtain a dynamic programming characterization of the upper and lower values of this zero-sum game. This dynamic program is obtained using the methodology described in Sections \ref{virtual} and \ref{sec:expanded}.


Consider a dynamic system with $M+N$ players. The players $1,\dots,M$ are in team 1 and the players $M+1, \dots, M+N$ are in team 2. The system operates in discrete time over a horizon $T$. Let $\rv{X}_t \in \X_t$ be the state of the system at time $t$, and let $\rv{U}_t^i \in \U_t^i$ be the action of player $i$ at time $t$, where $i = 1,\dots, M+N$. Let the actions of all the players at time $t$ be denoted by $\vec{U}_t := U_t^{1:M+N}$. The state of the system evolves in a controlled Markovian manner as
\begin{align}
\label{statevolteam}\rv{X}_{t+1} = f_t(\rv{X}_t, \vec{U}_t,\rv{W}_t^s),
\end{align}
where $\rv{W}_t^s$ is the system noise. There is an observation process $\rv{Y}_t^i \in \Y_t^i$ associated with each player $i$ and is given as
\begin{align}
\label{obseqteam}\rv{Y}_t^i = h_t^i(\rv{X}_t, \vec{U}_{t-1},\rv{W}_t^i), \; i = 1,\dots,M+N,
\end{align}
where $\rv{W}_t^i$ is an observation noise. We assume that the sets $\X_t, \U_t^i$ and $\Y_t^i$ are finite for all $i$ and $t$. Further,  the random variables $\rv{X}_1, \rv{W}_t^s, \rv{W}_t^i$ (referred to as \emph{the primitive random variables}) can take finitely many values and are mutually independent.

The collection of variables (i.e. observations, actions) available to player $i$ at time $t$ is denoted by $\rv{I}_t^i$. 
$\rv{I}_t^i$ is a subset of all observations until time $t$ and actions until $t-1$, i.e,   $ \rv{I}_t^i \subseteq \{\rv{Y}^{1:M+N}_{1:t}, \rv{U}^{1:M+N}_{1:t-1}\} $. The set of all possible realizations of $\rv{I}_t^i$ is denoted by $\mathcal{I}^i_t$. 

Information $\rv{I}_t^i$ can be decomposed into \emph{private} and \emph{common} information, i.e. $\rv{I}_t^i = \rv{C}_t \cup \rv{P}_t^i$. Common information $\rv{C}_t$ is the set of variables known to all the $M+N$ players at time $t$ while variables in the private information $\rv{P}_t^i$ are known only to player $i$. Let $\mathcal{C}_t$ be the set of all realizations of common information at time $t$ and let $\mathcal{P}_t^i$ be the set of all realizations of private information for player $i$ at time $t$.  We make the following assumption on the evolution of common and private information. This is similar to Assumption \ref{infevolve}. 

\begin{assumption}\label{infevolveteam}
The evolution of common and private information available to the players is as follows:
\begin{enumerate}
\item The common information $\rv{C}_t$ is increasing with time, i.e. $\rv{C}_t \subset \rv{C}_{t+1}$. Let $\rv{Z}_{t+1} := \rv{C}_{t+1}\setminus \rv{C}_t$ be the increment in common information. Thus, $\rv{C}_{t+1} = \{\rv{C}_t,\rv{Z}_{t+1}\}$. Furthermore,
\begin{align}
\label{commonevolteam}\rv{Z}_{t+1} = \zeta_{t+1}(\rv{P}_t^{1:M+N},\rv{U}_t^{1:M+N},\rv{Y}_{t+1}^{1:M+N}),
\end{align}
where $\zeta_{t+1}$ is a fixed transformation.
\item The private information evolves as
\begin{align}
\label{privevolteam}\rv{P}^i_{t+1} = \xi_{t+1}^i(\rv{P}_t^i,\rv{U}_t^i,\rv{Y}_{t+1}^i),
\end{align}
where $\xi_{t+1}^i$ is a fixed transformation.
\end{enumerate}
\end{assumption}
%As noted in \cite{nayyar2013decentralized} and \cite{nayyar2014common}, a number of information structures satisfy the above assumption.
%\red{Perhaps delete this}\textcolor{blue}{The first part of this assumption represents the increment in common information as a common observation set $\rv{Z}_{t+1}$ and states that $\rv{Z}_{t+1}$ can comprise of \emph{old} variables that were part of players' private information at time $t$ and \emph{new} variables generated at time $t$ and $t+1$, i.e. actions at $t$ and observations at $t+1$. The second part states that the evolution of each player's private information is influenced by their current private information and the new variables they generate.}

Players can use any information available to them to select their actions and we allow behavioral strategies for both players. Thus, player $i$ chooses a distribution $\delta\rv{U}_t^i$ over its action space using a \emph{control law} $g_t^i:  \mathcal{I}_t^i \rightarrow \Delta\mathcal{U}_t^i$, i.e.
\begin{equation}
\delta\rv{U}_t^i = g_t^i(\rv{I}_t^i) = g_t^i(\rv{P}_t^i,\rv{C}_t). \label{eq:stgteam}
\end{equation}
Player $i$'s action at time $t$ is randomly chosen from $\U_t^i$ according to the distribution $\delta\rv{U}_t^i$.

The collection of control laws $\vct{g}^i = (g_1^i,\dots,g_T^i)$ is referred to as the \emph{control strategy} of player $i$. Let the set of all possible control strategies for player $i$ be $\G^i$. The collection of strategies $g^1,\dots,g^M$ is referred to as the team profile of team 1 and is denoted by $\vec{g}^1$. Similarly, the collection of strategies $g^{M+1},\dots,g^{M+N}$ is referred to as the team profile of team 2 and is denoted by $\vec{g}^2$. The collection of control strategies $(\vct{g}^1,\dots,\vct{g}^{M+N})$ is referred to as a \emph{strategy profile} and is denoted by $(\vec{g}^1,\vec{g}^2)$. 

The total expected cost associated with a strategy profile $\vec{g}$ is
\begin{align}
J(\vec{g}^1,\vec{g}^2):=\E^{(\vec{g}^1,\vec{g}^2)}\left[\sum_{t=1}^T c_t(\rv{X}_t,\vec{U}_t)\right], \label{eq:totalcostteam}
\end{align}
where $c_t:\X_t \times \U_t^1 \times \dots \times  \U_t^{M+N} \rightarrow \R$ is the cost function at time $t$.
%\begin{align}
%J_m(\delta\vct{g}^1,\delta\vct{g}^2)= \sum_{\hat{\vct{g}}^1}\sum_{\hat{\vct{g}}^2}\delta\vct{g}^1(\hat{\vct{g}}^1)J(\hat{\vct{g}}^1,\hat{\vct{g}}^2)\delta\vct{g}^2(\hat{\vct{g}}^2).
%\end{align}
Each player $i$ in team 1, where $i = 1, \dots, M$, wants to minimize the total expected cost. And each player $i$ in team 2, where $i = M+1,\dots,M+N$, wants to maximize the total expected cost. We refer to this game as Game $\gm{T}$. 
\begin{definition}
The upper value of the game $\gm{T}$ is defined as
%\begin{align}
%S^u(\gm{T}) := \inf_{g^1,\dots,g^M}\sup_{g^{M+1},\dots,g^{M+N}} J(\vec{g}^1,\vec{g}^2).
%\end{align}
\begin{align}
S^u(\gm{T}) := \inf_{\vec{g}^1}\sup_{\vec{g}^2} J(\vec{g}^1,\vec{g}^2).
\end{align}
The lower value of the game $\gm{G}$ is defined as
%\begin{align}
%S^l(\gm{T}) := \sup_{g^{M+1},\dots,g^{M+N}} \inf_{g^1,\dots,g^M}J(\vec{g}).
%\end{align}
\begin{align}
S^l(\gm{T}) := \sup_{\vec{g}^2} \inf_{\vec{g}^1}J(\vec{g}^1,\vec{g}^2).
\end{align}
If the upper and lower values are the same,  they are referred to as  the value of the game and denoted by $S(\gm{T})$.   
\end{definition}
A Nash equilibrium among teams of the zero-sum game is a strategy profile $(\vec{g}^{1*},\vec{g}^{2*})$ such that for every team profile $\vec{g}^1$ for team 1 and every team profile $\vec{g}^2$ for team 2, we have
\begin{align}
J(\vec{g}^{1*},\vec{g}^{2}) \leq J(\vec{g}^{1*},\vec{g}^{2*}) \leq J(\vec{g}^{1},\vec{g}^{2*}).
\end{align}
%Nash equilibria in zero-sum games satisfy the following property \cite{osborne1994course}.
%\begin{proposition}
%If a Nash equilibrium in Game $\gm{G}$ exists, then for every Nash equilibrium $(\vct{g}^{1*},\vct{g}^{2*})$ in Game $\gm{G}$, we have
%\begin{align}
%J(\vct{g}^{1*},\vct{g}^{2*}) = S^l(\gm{G}) = S^u(\gm{G}) = S(\gm{G}).
%\end{align}
%%This equilibrium cost $S(\gm{G})$  is referred to as the value of the game.
%\end{proposition}
